An Analysis of Elo Rating Systems via Markov Chains

We present a theoretical analysis of the Elo rating system, a popular method for ranking skills of players in an online setting. In particular, we study Elo under the Bradley--Terry--Luce model and, using techniques from Markov chain theory, show that Elo learns the model parameters at a rate competitive with the state of the art. We apply our results to the problem of efficient tournament design and discuss a connection with the fastest-mixing Markov chain problem.

==> secs/proofs.tex <==
\section{Outline of Elo-Convergence Proofs}
\label{sec:proofs}


